3DiffTection: 3D Object Detection with Geometry-Aware Diffusion Features

We present 3DiffTection, a state-of-the-art method for 3D object detection from single images, leveraging features from a 3D-aware diffusion model. Annotating large-scale image data for 3D detection is resource-intensive and time-consuming. Recently, pretrained large image diffusion models have become prominent as effective feature extractors for 2D perception tasks. However, these features are initially trained on paired text and image data, which are not optimized for 3D tasks, and often exhibit a domain gap when applied to the target data. Our approach bridges these gaps through two specialized tuning strategies: geometric and semantic. For geometric tuning, we fine-tune a diffusion model to perform novel view synthesis conditioned on a single image, by introducing a novel epipolar warp operator. This task meets two essential criteria: the necessity for 3D awareness and reliance solely on posed image data, which are readily available (e.g., from videos) and does not require manual annotation. For semantic refinement, we further train the model on target data with detection supervision. Both tuning phases employ ControlNet to preserve the integrity of the original feature capabilities. In the final step, we harness these enhanced capabilities to conduct a test-time prediction ensemble across multiple virtual viewpoints. Through our methodology, we obtain 3D-aware features that are tailored for 3D detection and excel in identifying cross-view point correspondences. Consequently, our model emerges as a powerful 3D detector, substantially surpassing previous benchmarks, e.g., Cube-RCNN, a precedent in single-view 3D detection by 9.43\% in AP3D on the Omni3D-ARkitscene dataset. Furthermore, 3DiffTection showcases robust data efficiency and generalization to cross-domain data.

==> image_text/corresponding_result.tex <==
\begin{figure*}[t]
  \centering
  \label{fig:corr_results}
  \includegraphics[width=.97\linewidth, trim=10 0 10 0,clip]{figs/corres_exp.pdf}
  \caption{Novel-view synthesis results. The images are from the test set of ARkitscenes dataset, which are never seen by our proposed geometry ControlNet during training. }

\end{figure*}

==> tables/Pre-training-finetunehead.tex <==
\begin{table*}
\centering
  % \vspace{-3em}
  \caption{Read-Out experiments for pre-trained backbone. Note that we do not tune semantic controlnet}
\label{tab:readout}
% \tiny
\resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{1pt}
\begin{tabular}{l|c|c|c|c|c|c|c} 
% \begin{tabular}{ p{25mm}<{\centering}| p{10mm}<{\centering} | p{12mm}<{\centering}  p{10mm}<{\centering}  p{10mm}<{\centering} p{10mm}<{\centering} p{10mm}<{\centering} p{12mm}<{\centering} | p{10mm}<{\centering}}

\toprule
\textbf{Methods} & \textbf{Pre\-training} & \textbf{Backbone} & \textbf{Tuned Param.} & \textbf{AP3D}$\uparrow$ & \textbf{AP3D@15}$\uparrow$  & \textbf{AP3D@25}$\uparrow$ & \textbf{AP3D@50}$\uparrow$  \\
\midrule
CubeRCNN-VIT-B & MAE-pretrain    & ViT & 3D Head & 25.23  & 36.04 & 28.64 & 8.11\\
DreamTchr-Res50 & StableDiff distll.& Res50 & 3D Head& 24.36 & 34.16  & 25.97 & 7.93 \\
DIFT-SD        & StableDiff      & SD & 3D Head & 28.86 &  40.18 & 32.07 & 8.86 \\
\rowcolor[gray]{.9}
% DIFT-SD-Contr & Arktscn denoise.& SD+IVS-Contr & 3D Head &  
 % 26.05 & 35.81 & 29.86 & 6.95\\
\rowcolor[gray]{.9}
3DiffTection (w/o semantic-Contr) & Arktscn nvs.    &  SD+NVS-Contr & 3D Head & 31.20 & 41.87 & 33.53 &  10.14 \\
% \rowcolor[gray]{.9}
% 3DiffTection   & Arktscn nvs.    & 512$\times512$ & 3D Head &  &  &  & \\
\bottomrule
\end{tabular}
}
\end{table*}
